Learning to Impute: A General Framework for Semi-supervised Learning

Recent semi-supervised learning methods have shown to achieve comparable results to their supervised counterparts while using only a small portion of labels in image classification tasks thanks to their regularization strategies. In this paper, we take a more direct approach for semi-supervised learning and propose learning to impute the labels of unlabeled samples such that a network achieves better generalization when it is trained on these labels. We pose the problem in a learning-to-learn formulation which can easily be incorporated to the state-of-the-art semi-supervised techniques and boost their performance especially when the labels are limited. We demonstrate that our method is applicable to both classification and regression problems including image classification and facial landmark detection tasks.

==> alg1.tex <==

\begin{algorithm}[H]
    \SetAlgoLined
	\footnotesize
	\KwIn{$T$, $\mathcal{U}$ \Comment*[f]{ $T$ indicates the training set, $\mathcal{U}$ is the unlabeled set}}
	\textbf{Required}: model function $\Phi$ and its initialization parameters $\theta^0$, a batch of training data $\mathcal{B}_t^{T}=\{\bx_i, y_i\}_{i=1, \cdots, |\mathcal{B}_t^{T}|}$, a batch of unlabeled data $\mathcal{B}_t^{\mathcal{U}}=\{\bx_i^{\mathcal{U}}\}_{i=1, \cdots, |\mathcal{B}_t^{\mathcal{U}}|}$ and another batch of training data (treated as validation data during training) $\mathcal{B}_t^{V}=\{\bx_i, y_i\}_{i=1, \cdots, |\mathcal{B}_t^{V}|}$ and learning rate $\alpha, \eta, \eta_z$\\
    % \textbf{for} t in range(K) \textbf{do} {\rightline $\rhd$ K indicates the total number of training epochs} \\
    % \textbf{for} $t$ in range($K$)
    % \Comment*[f]{$K$ indicates the total number of training epochs}\\
	\For{$t = 0, \cdots, K-1$}
	{
	   % sample a batch of training data $\mathcal{B}_t^{T}=\{\bx_i, y_i\}_{i=1, \cdots, |\mathcal{B}_t^{T}|}$;\\
	   % sample a batch of unlabeled data
	   % $\mathcal{B}_t^{\mathcal{U}}=\{\bx_i^{\mathcal{U}}\}_{i=1, \cdots, |\mathcal{B}_t^{\mathcal{U}}|}$;\\
	   % sample another batch of training data $\mathcal{B}_t^{V}=\{\bx_i, y_i\}_{i=1, \cdots, |\mathcal{B}_t^{V}|}$;\\
	    $\bz = \{z_i\}_{i=1, \cdots, |\mathcal{B}_t^{\mathcal{U}}|} = \{\Phi_{\theta^t}(\bx_i^{\mathcal{U}})\}_{i=1, \cdots, |\mathcal{B}_t^{\mathcal{U}}|}$; \Comment*[f]{ estimate pseudo labels for unlabeled samples}\\
	    
	    $\mathcal{C}^{A}=\sum_{i=1}^{|\mathcal{B}_t^{T}|}\ell(\Phi_{\theta^t}(\bx_i), y_i)+\lambda \sum_{i=1}^{|\mathcal{B}_t^{\mathcal{U}}|}\ell(\Phi_{\theta^t}(\bx_i^{\mathcal{U}}), z_i)$;\\
	    
	    $\hat{\theta}^{t} = \theta^t - \eta \frac{d \mathcal{C}^{A}}{d \theta^t}$;\Comment*[f]{update the model and move to the meta update}\\
	    
	    
	    $\bz = \{z_i\}_{i=1, \cdots, |\mathcal{B}_t^{\mathcal{U}}|} = \{\Phi_{\hat{\theta}^{t}}(\bx_i^{\mathcal{U}})\}_{i=1, \cdots, |\mathcal{B}_t^{\mathcal{U}}|}$;\Comment*[f]{ estimate pseudo labels using the updated model}\\
	    
	    $\mathcal{C}=\sum_{i=1}^{|\mathcal{B}_t^{\mathcal{U}}|}\ell(\Phi_{\hat{\theta}^{t}}(\bx_i^{\mathcal{U}}), z_i)$;\\
	    
	    $\hat{\theta}^{t+1}=\hat{\theta}^{t} - \alpha \frac{d \mathcal{C}}{d \hat{\theta}^{t}}$;\Comment*[f]{simulate a step}\\
	    
	    
	    $\mathcal{C}^{V}(\hat{\theta}^{t+1})=\sum_{i=1}^{|\mathcal{B}_t^{V}|}\ell(\Phi_{\hat{\theta}^{t+1}}(\bx_i), y_i)$; \Comment*[f]{evaluate on validation data}\\
	    
	    $\hat{\bz} = \bz - \eta_z \frac{d \mathcal{C}^{V}}{d \bz}$; \Comment*[f]{\color{cyan} correct pseudo labels}\\
	    $\hat{\mathcal{C}}= \sum_{i=1}^{|\mathcal{B}_t^{\mathcal{U}}|}\ell(\Phi_{\theta_t}(\bx_i^{\mathcal{U}}), \hat{z}_i)$;\\
	    
	   % $L^V = L^{CE}(\Phi_{\hat{\theta}_{t+I}}, \mathcal{B}_t^{V})$;\\
	   
	    $\theta^{t+1} = \hat{\theta}^t - \eta  \frac{d \hat{\mathcal{C}}}{d \hat{\theta}^{t}}$ \Comment*[f]{\color{cyan} update the model with corrected pseudo labels}
	    
    }
	\KwOut{$\theta^{K}$}
	\caption{Option1}\label{algorithm:Option1}
\end{algorithm}

==> alg2.tex <==

\begin{algorithm}[htp]
	\footnotesize
	\caption{Option2}\label{algorithm:Option2}
	\KwIn{$T, \mathcal{U}$\Comment*[f]{ $T$ indicates the training set, $\mathcal{U}$ is the unlabeled set}}
	\textbf{Required}: model function $\Phi$ and its initialization parameters $\theta^0$, a batch of training data $\mathcal{B}_t^{T}=\{\bx_i, y_i\}_{i=1, \cdots, |\mathcal{B}_t^{T}|}$, a batch of unlabeled data $\mathcal{B}_t^{\mathcal{U}}=\{\bx_i^{\mathcal{U}}\}_{i=1, \cdots, |\mathcal{B}_t^{\mathcal{U}}|}$ and another batch of training data (treated as validation data during training) $\mathcal{B}_t^{V}=\{\bx_i, y_i\}_{i=1, \cdots, |\mathcal{B}_t^{V}|}$ and learning rate $\alpha, \eta$\\
	\For{$t = 1, \cdots, K-1$}
	{
	   % sample a batch of training data $\mathcal{B}_t^{T}=\{\bx_i, y_i\}_{i=1, \cdots, |\mathcal{B}_t^{T}|}$;\\
	   % sample a batch of unlabeled data
	   % $\mathcal{B}_t^{\mathcal{U}}=\{\bx_{i}^{\mathcal{U}}\}_{i=1, \cdots, |\mathcal{B}_t^{\mathcal{U}}|}$;\\
	   % sample another batch of training data $\mathcal{B}_t^{V}=\{\bx_i, y_i\}_{i=1, \cdots, |\mathcal{B}_t^{V}|}$;\\
	    
	    $\bz = \{z_i\}_{i=1, \cdots, |\mathcal{B}_t^{\mathcal{U}}|} = \{\Phi_{\theta^t}(\bx_{i}^{\mathcal{U}})\}_{i=1, \cdots, |\mathcal{B}_t^{\mathcal{U}}|}$;\Comment*[f]{ estimate pseudo labels for unlabeled samples}\\
	    
	    $\mathcal{C}^{A}=\sum_{i=1}^{|\mathcal{B}_t^{T}|}\ell(\Phi_{\theta^t}(\bx_i), y_i)+\lambda \sum_{i=1}^{|\mathcal{B}_t^{\mathcal{U}}|}\ell(\Phi_{\theta^t}(\bx_{i}^{\mathcal{U}}), z_i)$;\\
	    
	    $\hat{\theta}^{t} = \theta^t - \eta \frac{d \mathcal{C}^{A}}{d \theta^t}$;\Comment*[f]{update the model and move to the meta update}\\

	    $\bz = \{z_i\}_{i=1, \cdots, |\mathcal{B}_t^{\mathcal{U}}|} = \{\Phi_{\hat{\theta}^{t}}(\bx_{i}^{\mathcal{U}})\}_{i=1, \cdots, |\mathcal{B}_t^{\mathcal{U}}|}$;\Comment*[f]{estimate pseudo labels using the updated model}\\
	    
	    $\mathcal{C}=\sum_{i=1}^{|\mathcal{B}_t^{\mathcal{U}}|}\ell(\Phi_{\hat{\theta}^{t}}(\bx_{i}^{\mathcal{U}}), z_i)$;\\
	    
	    $\hat{\theta}^{t+1}=\hat{\theta}^{t} - \alpha \frac{d \mathcal{C}}{d \hat{\theta}^{t}}$;\Comment*[f]{simulate a step}\\
	       % $L_{i} = L^{Con}(\Phi_{\hat{\theta}_t}, \mathcal{B}_t^{\mathcal{U}})$;\\
	       % $\hat{\theta}_{t+i} = \hat{\theta}_{t+i-1} - \eta * \frac{d L_{i}}{d \hat{\theta}_{t+i-1}}$;\\
	       
	    $\mathcal{C}^{V}(\hat{\theta}^{t+1})=\sum_{i=1}^{|\mathcal{B}_t^{V}|}\ell(\Phi_{\hat{\theta}^{t+1}}(\bx_i), y_i)$;\Comment*[f]{evaluate the simulated step on validation data}\\
	    
	    $\theta^{t+1} = \hat{\theta}^t - \eta \frac{d \mathcal{C}^{V}}{d \hat{\theta}^{t}}$;\Comment*[f]{\color{cyan} derive the meta gradient on the model and update the model directly}\\
	    
	}
	\KwOut{$\theta^{K}$}
\end{algorithm}

==> broim.tex <==
It is well recognized that large-scale labeled datasets are one of the driving forces in the success of deep learning models.
However, while manual labeling of data can be done efficiently with crowdsourcing, it is still an expensive and tedious process that hinders a widespread adoption of machine learning methods in different fields such as medical imaging.
Given that our method performs better than the existing methods in low label regime and can be used in both classification and regression, it can potentially be used in many machine learning applications such as cancer tissue segmentation from medical images, landslide and earthquake damage estimation from satellite images where it is challenging and expensive to obtain labeled data.

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> method_old.tex <==
% !TEX root = main.tex
Consider a dataset $\mathcal{D}$ that consists of $|\mathcal{L}|$ labeled samples $\mathcal{L}=\{(\bx_1,\by_1),(\bx_2,\by_2),\dots,(\bx_{|\mathcal{L}|},\by_{|\mathcal{L}|})\}$ which is further split into a training $\mathcal{T}$ and meta-validation set $\mathcal{V}$ with $|\mathcal{T}|$ and $|\mathcal{V}|$ samples respectively.
We also have a set of unlabeled samples $\mathcal{U}=\{\bx^{u}\}_{i=1,\dots, |\mathcal{U}|}$. 
Further, we let $\Phi_\theta$ denote a model (a function parameterized for instance, as a deep neural network) with parameters $\theta$, that is trained to predict labels $y$ from given samples $x$ as $\by = \Phi_\theta(\bx)$.
%Furthermore, let $\by = \Phi_\theta(\bx)$ be a model such as a deep neural network whose parameters $\theta$ are optimized to predict labels from samples.

% \input{alg}

We are interested in imputing missing labels $\bz$ of the unlabeled samples that are not only accurate but also improve performance at inference time, when included in our training set for optimizing model parameters $\theta$.
A straightforward approach to this problem is to first train a model to optimize the following cost function on the training set $\mathcal{T}$:
\begin{equation}\label{e:costL}
\arg\min_{\theta}\sum_{\bx\in \mathcal{T}} \ell(\Phi_\theta(\bx),\by)
\end{equation} where $\ell$ is a task specific loss, such as a soft-max followed by a cross-entropy loss for classification or squared loss for regression tasks.

%can be designed as a soft-max followed by a cross entropy loss for classification or sum of square distances for regression tasks.

\paragraph{\whicml{Conventional Approaches.}}
One can then use the trained model $\Phi_\theta$ to impute labels for samples in the unlabeled set $\mathcal{U}$ as \wh{$\bz=\Phi_\theta(\tilde{\bx}^u)$ as in \cite{tarvainen2017mean,berthelot2019mixmatch}, where $\tilde{\bx}^u$ denotes randomly perturbed input image $\bx^{u}$ (\eg random crops). Note that the label imputation procedure can be replaced with other pseudo-label prediction techniques.}

Now we can expand $\mathcal{T}$ by adding the unlabeled samples with their imputed pseudo-labels \ie $\mathcal{A}=\mathcal{T} \cup \mathcal{U}$ and further train $\theta$ by using \cref{e:costL}.
However, as many pseudo-labels $\bz$ will likely be noisy, there is no guarantee that training on the augmented train set will improve the performance of the model on the meta-validation set $\mathcal{V}$:
\begin{equation}\label{e:costV}
C^V=\sum_{\bx\in\mathcal{V}} \ell(\Phi_\theta(\bx),\by).
\end{equation} Note that in all our experiments $\mathcal{V}$ is randomly sampled from $\mathcal{T}$ which ensures that our method is not trained using any additional data.

\paragraph{\whicml{Our Method: Learning to Impute.}}
Our goal is also to minimize the expected value of the loss in \cref{e:costL} with respect to the model parameters $\theta$ via an algorithm such as stochastic gradient descent (SGD).
Here, we go a step further and consider how the label imputation affects the ability of SGD to optimize the loss in \cref{e:costV}.


\begin{figure*}[t]
	\centering
% include first image
	\includegraphics[width=.7\linewidth]{./figures/ToyCircles.pdf}  
	\includegraphics[width=.7\linewidth]{./figures/ToyCirclesUn.pdf}
	\caption{Results on the toy binary classification task. The top and bottom rows correspond to the predictions on the test and unlabeled data respectively. Points in {\color{green} green} and {\color{pink} pink} are labeled training samples. Best seen in color.}
	\label{fig:circles}
\end{figure*}

We pose this as a meta-learning problem, which is derived next.
We start by considering the loss value of the model $\Phi_\theta$ on the augmented training set $\mathcal{A}$:
\begin{equation}\label{e:lossA}
  \mathcal{C}^A =\sum_{\bx\in\mathcal{T}}\ell(\Phi_\theta(\bx), \by) + \sum_{\bx^u\in\mathcal{U}}\ell(\Phi_\theta(\bx^u), \bz).
\end{equation}
\whicml{Instead of directly using the pseudo-labels $\bz=\Phi_\theta(\tilde{\bx}^u)$, we first simulate a step of SGD using the loss of unlabeled images, $\mathcal{C}=\sum_{\bx^u\in\mathcal{U}}\ell(\Phi_\theta(\bx^u), \bz)$ to drive the update of the model parameters $theta$.}
% We first simulate a step of SGD using the loss in \cref{e:lossA} to drive the update of the model parameters $\theta$.
At step $t$, SGD updates the parameters \whicml{for minimizing $\mathcal{C}=\sum_{\bx^u\in\mathcal{U}}\ell(\Phi_\theta(\bx^u), \bz)$ as follows:}
% a given $\bx^{u}\in\mathcal{U}$ as follows:
\begin{equation}\label{e:sgdupdate}
\begin{small}
\whicml{\hat{\theta}^{t+1} = \theta^t - \eta \nabla_\theta \left(\sum_{\bx^u\in\mathcal{U}}\ell(\Phi_\theta(\bx^u), \bz)\right),}
  % \wh{\hat{\theta}^{t+1} = \theta^t - \eta \nabla_\theta \left(\sum_{\bx\in\mathcal{T}}\ell(\Phi_\theta(\bx), \by) + \sum_{\bx^u\in\mathcal{U}}\ell(\Phi_\theta(\bx^u), \bz)\right),}
\end{small}
\end{equation}
% \begin{equation}\label{e:sgdupdate}
%   \hat{\theta}^{t+1} = \theta^t - \eta \nabla_\theta \ell(\Phi_{\theta^t}(\bx^{u}),\bz^t)
% \end{equation}
where $\nabla_\theta$ is the gradient operator. \wh{We then wish to find $\bz$ that minimizes the meta-validation objective $C^V(\hat{\theta}^{t+1})$ in \cref{e:costV} with $\hat{\theta}^{t+1}$. This corresponds to the following bilevel optimization problem}
% Now we can re-write \cref{e:costV} with $\hat{\theta}^{t+1}$:
\whicml{\begin{equation}\label{e:costVtheta}
\begin{small}
\begin{aligned}
&\min_{\bz} \left(\sum_{\bx \in \mathcal{V}} \ell(\Phi_{\hat{\theta}^{t+1}}(\bx),\by)\right),\\
&\text{subject to}~\hat{\theta}^{t+1} = \theta^t - \eta \nabla_\theta \left(\sum_{\bx^u\in\mathcal{U}}\ell(\Phi_\theta(\bx^u), \bz)\right).
  % \wh{\min_{\bz} \left(\sum_{\bx \in \mathcal{V}} \ell(\Phi_{\hat{\theta}^{t+1}}(\bx),\by)\right),~\text{subject to}~\hat{\theta}^{t+1} = \theta^t - \eta \nabla_\theta \left(\sum_{\bx\in\mathcal{T}}\ell(\Phi_\theta(\bx), \by) + \sum_{\bx^u\in\mathcal{U}}\ell(\Phi_\theta(\bx^u), \bz)\right).}
\end{aligned}
\end{small}
\end{equation}}Our goal \whicml{of optimizing \cref{e:costVtheta}} is to learn predicted pseudo-labels that minimize the \wh{meta-validation} loss in \cref{e:costVtheta}. To this end, we propose two options, denoted as \textbf{Option 1} and \textbf{Option 2}. In the former, we treat $\bz$ as latent (or learnable) parameters \wh{and} compute the gradients of the \wh{meta-validation} loss w.r.t $\bz$ to update$\bz$, \wh{which is used to update model parameters $\theta$.} In the latter, $\bz$ is considered as the output of network $\Phi_{\theta}$ \wh{and} the gradients are thus computed w.r.t the model parameters $\theta$ \wh{for updating $\theta$.}
% and used to update $\theta$. 
% \begin{equation}\label{e:costVtheta}
%   C^V(\hat{\theta}^{t+1}) = \sum_{\bx \in \mathcal{V}} \ell(\Phi_{\hat{\theta}^{t+1}}(\bx),\by).
% \end{equation} 


% \paragraph{Discussion.} Note that naively setting the pseudo-labels to the output of the network (\ie $\bz=\Phi_{\theta}(\bx^u)$) yields zero loss and thus no gradient for $\ell(\Phi_\theta(\bx^u), \bz)$ in \cref{e:lossA}.
% Non-zero loss can be achieved by injecting stochasticity to the pseudo-label prediction which can be realized in several ways such as using drop-out layers in the network, adding random perturbations to the input ($\bx^u$)  and/or output of the network ($\Phi_\theta$).
% As a matter of fact, we use different random crops of input images to compute the output and pseudo-labels when our inputs are images.
% % We denote the random cropping operation as $\Omega$.
% In the toy experiments, where the input samples are $2$-d points, we use the Gumbel-softmax function \cite{jang2017categorical} to compute the pseudo-labels, as it outputs hard-labels (or one-hot probabilities) in a differentiable manner.


\paragraph{Optimization.}
The gradients of $C^V$ w.r.t $\bz$ for Option 1 and w.r.t $\theta$ for Option 2 are respectively be written as:
%\begin{equation}\label{e:upz}
%\frac{\partial{C}^V}{\partial {\bz}} = \left(\sum_{\bx\in\mathcal{V}} \frac{\partial \ell(\Phi_{\hat{\theta}^{t+1}}(\bx), \by)}{\partial \Phi_{\hat{\theta}^{t+1}}(\bx)} \cdot \frac{\partial \Phi_{\hat{\theta}^{t+1}}(\bx)}{\partial \hat{\theta}^{t+1}}\right) \cdot \frac{\partial \hat{\theta}^{t+1}}{\partial {\bz}}  
%\end{equation} where $\partial\hat{\theta}^{t+1}/\partial \bz^t$ can be derived by plugging in \cref{e:sgdupdate} for Option 1:
%\begin{equation}\label{e:dtdz}
%\frac{\partial \hat{\theta}^{t+1}}{\partial {\bz}} = \frac{\partial \theta^t}{\partial \bz} - \eta \nabla_z \nabla_{\theta} \ell(\Phi_{\theta}(\bx^{u}), \bz^t).
%\end{equation}
%\begin{equation}\label{e:dzdt}
%\frac{d \theta^t}{d z} = 0.
%\end{equation}
%Similarly, $\partial\hat{\theta}^{t+1}/\partial \theta^t$ can be written as:
%\begin{equation}\label{e:dtdt}
%\frac{\partial \hat{\theta}^{t+1}}{\partial {\theta^t}} = \mathcal{I} - \eta \nabla_{\theta} \nabla_{\theta} \ell(\Phi_{\theta}(\bx^{u}), \bz^t)
%\end{equation} where $\mathcal{I}$ is identity matrix and $\nabla_{\theta} \nabla_{\theta}$ requires a second order derivative computation which is computed approximately.
%Plugging \cref{e:dtdz} into \cref{e:upz} gives
% \begin{small}
% \begin{align}
% \label{e:upfinal1}
% \wh{(\textbf{Option 1})}~~\frac{\partial{C}^V}{\partial \bz} & = \left(\sum_{\bx\in\mathcal{V}} \frac{\partial \ell(\Phi_{\hat{\theta}^{t+1}}(\bx), \by)}{\partial \hat{\theta}^{t+1}}\cdot \frac{\partial \Phi_{\hat{\theta}^{t+1}}(\bx)}{\partial \hat{\theta}^{t+1}}\right) \cdot \left(\frac{\partial \theta^t}{\partial \bz}- \eta \nabla_{\bz}\nabla_\theta \wh{\mathcal{C}^A} \right)\\
% \label{e:upfinal2}
% \wh{(\textbf{Option 2})}~~\frac{\partial{C}^V}{\partial \theta^t} & = \left(\sum_{\bx\in\mathcal{V}} \frac{\partial \ell(\Phi_{\hat{\theta}^{t+1}}(\bx), \by)}{\partial \hat{\theta}^{t+1}}\cdot \frac{\partial \Phi_{\hat{\theta}^{t+1}}(\bx)}{\partial \hat{\theta}^{t+1}}\right) \cdot \left(\wh{\frac{\partial \theta^t}{\partial \bz} \frac{\partial \bz}{\partial \theta^t}- \eta \nabla_{\theta} \nabla_{\theta} \mathcal{C}^A}\right)
% \end{align}\end{small}where 
% % $\mathcal{I}$ is identity matrix and 
% $\nabla_{\theta} \nabla_{\theta}$ indicates a second order derivative which is supported by standard deep learning libraries such as Pytorch~\cite{paszke2017automatic}, Tensorflow~\cite{tensorflow2015-whitepaper}.
\whicml{\begin{small}
\begin{align}
\label{e:upfinal1}
\wh{(\textbf{Option 1})}~ \frac{\partial{C}^V}{\partial \bz} & = \sum_{\bx\in\mathcal{V}} \frac{\partial \ell(\Phi_{\hat{\theta}^{t+1}}(\bx), \by)}{\partial \hat{\theta}^{t+1}}\cdot \left(\frac{\partial \theta^t}{\partial \bz}- \eta \nabla_{\bz}\nabla_\theta \wh{\mathcal{C}} \right),\\
\label{e:upfinal2}
\wh{(\textbf{Option 2})}~ \frac{\partial{C}^V}{\partial \theta^t} 
% & = \frac{\partial{C}^V}{\partial \bz}\frac{\partial{\bz}}{\partial \theta^t} 
&= \sum_{\bx\in\mathcal{V}} \frac{\partial \ell(\Phi_{\hat{\theta}^{t+1}}(\bx), \by)}{\partial \hat{\theta}^{t+1}} \cdot \left(\wh{\mathcal{I}- \eta \nabla_{\theta} \nabla_{\theta} \mathcal{C}}\right),
\end{align}\end{small}}where 
$\mathcal{I}$ is identity matrix and
$\nabla_{\theta} \nabla_{\theta}$ indicates a second order derivative which is supported by standard deep learning libraries such as Pytorch~\cite{paszke2017automatic}, Tensorflow~\cite{tensorflow2015-whitepaper}.
 % \wh{and $\frac{\partial \theta^t}{\partial \bz}=0$ as $\theta^t$ is not a function of $\bz$}.

\wh{We then use the gradients in \cref{e:upfinal1} or \cref{e:upfinal2} to update the model parameters such that the updated model can predict pseudo-labels that minimize the meta-validation loss. In Option 1, we update the pseudo-labels as $\hat{\bz}=\bz - \eta_z \frac{d \mathcal{C}^{V}}{d \bz}$ and the updated pseudo-labels are then used to update the model parameters $\theta$ by minimizing the loss $\mathcal{C}^{U}= \sum_{\bx^u\in\mathcal{U}}\ell(\Phi_{\theta_t}(\bx_i^{u}), \hat{z}_i)$. In Option 2, the gradient in \cref{e:upfinal2} is used to update the model parameters as $\theta^{t+1}=\theta^{t}-\eta\frac{\partial \mathcal{C}^{V}}{\partial \theta^{t}}$}



We further depict the optimization details of Option 1 and 2 in Alg.~\ref{algorithm:option12}. 
We first estimate the $\bz$ with the current model $\theta^t$, update the model to optimize the loss $\mathcal{C}^{A}$ and then re-estimate $\bz$ with $\hat{\theta}^{t}$. 
This part is so far similar to the self-labeling method of~\cite{lee2013pseudo}. 
% CS: What does the It in "It can trivially.." refer to? The loss?
The loss function $\mathcal{C}^{A}$ can trivially be replaced by those used in recent work such as Mean-Teacher~\citep{tarvainen2017mean} or MixMatch~\citep{berthelot2019mixmatch};
we applied our method in conjunction with all three loss functions and report results in \cref{s:exp}.
%In fact, we incorporate our method to these three techniques and report results in \cref{s:exp}.
Next we apply the updated model to a mini-batch of unlabeled samples, compute the loss and simulate a SGD step w.r.t this loss. 
\wh{In Option 1, we initialize $z$ with the output of $\Phi_\theta(\tilde{\bx}^u)$ and update it by using the gradient from \cref{e:upfinal1}.}
 % where $\tilde{\bx}^u$ denotes randomly perturbed input image $\bx^u$ (\ie random crop).}
% The updated pseudo-label $\hat{\bz}=\bz - \eta_z \frac{d \mathcal{C}^{V}}{d \bz}$ is then used to update the model $\theta$ by minimizing the loss $\hat{\mathcal{C}}= \sum_{\bx^u\in\mathcal{U}}\ell(\Phi_{\theta_t}(\bx_i^{u}), \hat{z}_i)$.
In Option 2, the meta-update is computed w.r.t $\theta$ and used to update the model parameters by using the gradient from \cref{e:upfinal2}.
% : $\theta^{t+1} = \hat{\theta}^t - \eta \frac{\partial \mathcal{C}^{V}}{\partial \theta}$.



%\paragraph{Option 1: $\bz$ as latent parameters.} In this case, we create a $\bz$ vector for each $\bx^u$, initialize $z^{t=0}$ with the output of $\Phi_\theta^{t=0}(\bx)$ and update it by using the gradient from \cref{e:upfinal}. In case of classification, the pseudo-labels are obtained after applying a gumbel-softmax~\cite{jang2017categorical} on the original $\bz$ in the toy experiment or a softmax on jittered input (\eg random cropping) in the image classification and regression experiments. Here we assume that $\frac{d \theta^t}{d \bz}=0$, as $\theta$ is not a function of $\bz$. 
%
%\paragraph{Option 2: $\bz$ as output of model $\Phi$.} In this case, $\bz$ is computed from the network's output, \ie $\bz=\sigma(\Phi_\theta)$ where $\sigma$ can be a gumbel-softmax operator or softmax for classification. In contrast to option 1, $\bz$ is a function of $\Phi_{\theta}$ and thus $\theta$. The meta-update is computed w.r.t $\theta$ and used to update the model parameters, which involves (approximate) computation of second order derivatives.



==> relwork_old.tex <==
% !TEX root = main.tex
\subsection{Semi-supervised classification.}
There is a rich body of literature in SSL~\cite{chapelle2009semi} for classification.
Most of the recent work~\cite{lee2013pseudo,tarvainen2017mean,miyato2018virtual,berthelot2019mixmatch,xie2019unsupervised,sohn2020fixmatch,Berthelot2019ReMixMatchSL,Athiwaratkun2019ThereAM} builds on the idea of the bootstrapping technique of ~\cite{yarowsky1995unsupervised} that involves iterative optimization of classifier on a set of labeled data and refinement of its labels for the unlabeled data.
This paradigm is known to overfit on the noisy self-generated labels and thus suffer from low generalization performance.
To alleviate the sensitivity to inaccurate labeling, researchers introduce various regularization strategies.
\cite{grandvalet2005semi} proposes a minimum entropy regularizer that encourages each unlabeled sample to be assigned to only one of the classes with high probability.
\cite{lee2013pseudo} instead follows a more direct approach, use the predicted label with the maximum probability for each unlabeled sample as true-label which is called ``pseudo-label''.
An orthogonal regularization strategy is to encourage a classifier to be invariant to various stochastic factors and produce consistent predictions for unlabeled data when the noise is added to intermediate representations~\cite{srivastava2014dropout} and to input in an adversarial manner~\cite{miyato2018virtual}.
In the same vein, \cite{laine2016temporal,tarvainen2017mean} introduce the $\Pi$-model and Mean-Teacher that are regularized to be consistent over previous training iterations by using a temporal ensembling and teacher/student networks respectively.
Recently \cite{berthelot2019mixmatch} introduced MixMatch algorithm that further extends the previous work by unifying the idea of the consistency regularization and augmentation strategies \cite{zhang2018mixup}. Athiwaratkun et al. \cite{Athiwaratkun2019ThereAM} combine the $\Pi$-model and Mean-Teacher with the Stochastic Weight Averaging \cite{Izmailov2018AveragingWL} while \cite{Berthelot2019ReMixMatchSL,sohn2020fixmatch} extend the MixMatch using existing strong augmentation techniques (\eg RandAugment~\cite{cubuk2019randaugment}, AutoAugment~\cite{cubuk2019autoaugment}, Cutout~\cite{devries2017improved} etc.) to better regularize the network with unlabeled data.
% to formulate a new and simple method which regularizes the consistency of pseudo label estimated from a weakly augmented unlabeled image and the prediction of the strongly augmented one.
While the recent techniques are shown to be effective in several classification benchmarks, the idea of consistency regularization is still implicit in terms of generalization performance.
Here we take an orthogonal and more direct approach to this approach and learn to impute the labels of the unlabeled samples that improve the generalization performance of a classifier. We also show that our method can be used with the recent SSL techniques and for both classification and regression problems. 
% In contrast, \cite{laine2016temporal} introduce the $\Pi$ model exploiting the  stochasticity of the prediction function itself (i.e. the prediction model can produce different outputs for the same input) to apply consistency regularization to standard supervised learning framework. $\Pi$ model achieves this by adding a loss term to encourage the difference between a network's output for different passes of the same image to be small. This is shown to be efficient and effecitve on semi-supervised learning. However, as $\Pi$ model relies on a potentially unstable ``target” prediction, which can rapidly change during the course of training and the ``target'' prediction can be very noisy, the training process can be unstable. To tackle the difficulty with $\Pi$ model, \cite{tarvainen2017mean} propose Mean Teacher which exploits an exponential average update strategy to update a teacher network for ``target'' prediction. In Mean Teacher, the teacher network made via exponential average over the student network is supposed to include more reliable stochastic information and thus the ``target'' prediction is more confident. Similarly, \cite{berthelot2019mixmatch} also consider adding the consistency regularization to the network. The most distinction between the proposed MixMatch method and existing consistency regularization based methods (e.g., $\Pi$ model and mean teacher) is, MixMatch average the predictions of different augmentations and sharpen them to form the pseudo labels for the unlabeled images and exploiting the MixUp \cite{zhang2018mixup} to augment both the labeled and unlabeled images. With the labeled guessing and MixUp techniques introduced in the MixMatch, the semi-supervised learning performance on two popular image classification datasets is significantly boosted. 
% Different from $\Pi$ model and mean teacher replying on the stochasticity inside the network itself, \cite{miyato2018virtual} develop the Virtual Adversarial Training (VAT) which directly approximates a tiny perturbation radv added to the input which would most signiﬁcantly affect the output of the prediction model. 


% /***weihong adding reviews of label propagation approaches here***/

\subsection{Semi-supervised regression.}
Some of the recent techniques in semi-supervised classification are shown to be applicable to regression problems. \cite{jean2018semi} have adapted various existing SSL methods such as label propagation, VAT~\cite{miyato2018virtual} and Mean Teacher~\cite{tarvainen2017mean} and studied their performance in regression. The same authors also proposed a Bayesian SSL approach for SSL regression problems which is based on the recent deep kernel learning method~\cite{wilson2016deep} based approach for semi-supervised learning that aims at minimizing predictive variance of unlabeled data. As in the classification task, these methods are typically ad-hoc and does not aim to generate labels for the unlabeled data that are optimized to improve the generalization in regression.


% Different from these methods for both classification or regression tasks, our proposed method aims at learning the model to automatically and more correctly label unlabeled images. Instead of directly use the current function/model to predict the ``targets'' or pseudo labels for unlabeled data, we consider exploiting the supervision signal from the validation data to correct those wrong/noisy ``targets''/pseudo labels for unlabeled data. This enables our method to train the network with more reliable generated supervision signals of unlabeled data and thus boosts the semi-supervised learning performance on both the classification and regression tasks.

\subsection{Meta-learning.}
Our method is also related to meta-learning~\cite{schmidhuber1987evolutionary,bengio1992optimization,Hospedales2020MetaLearningIN} and inspired from the recent work~\cite{andrychowicz2016learning,finn2017model} where the goal is typically to quickly learn a new task from a small amount of new data. \cite{andrychowicz2016learning,finn2017model} propose a learn gradient through gradient approach to train a model which has a strong generalization ability to unseen test data and can be easily adapted to new/unseen tasks. \cite{sung2018learning} introduce the relation network to learn an additional metric such that the learned model's feature embedding can be generalized for unseen data and unseen tasks. 
\cite{ren2018learning} adopt the meta learning to learn the weight of samples to tackle the sample imbalance problem.
\cite{lorraine2018stochastic,mackay2019self} employ meta learning for automatically learning the hyper-parameters of the deep neural networks. 
Meta-learning has recently been applied to unsupervised learning \cite{hsu2018unsupervised} and SSL for few shot learning \cite{ren2018meta}. 
\cite{ren2018meta} adapts the prototypical network to use unlabeled examples when producing prototypes, enabling the prototypical network to exploit those unlabeled data to assist few shot classification. 
\cite{Antoniou2019critique} propose to learn a label-free loss function, parameterized as a neural network that enables the classifier to leverage the information from a validation set and achieves better performance in few-shot learning.
\cite{sun2019learning} propose a meta-learning technique to initialize a self-training model and to filter out noisy pseudo labels for semi-supervised few-shot learning.
Similarly, our work also builds on the ideas of optimizing for improving the generalization for unseen samples.
However, in contrast to the existing meta-learning methods that is proposed for few-shot learning problems, we focus on semi-supervised learning in general classification and regression problems where the number of samples are not limited to few.


% we mainly focus on developing meta learning approach for  Our method is learned to more correctly label unlabeled image to assist the training of deep neural network. Also, our method is suitable for both classification and regression tasks.

==> scratch.tex <==

\noindent \textbf{Semi-supervised classification.} \cite{grandvalet2005semi} motivate minimum entropy regularization so as to incorporate unlabeled data in the standard supervised learning. \cite{lee2013pseudo} estimate the class probability of an unlabeled image and pick up the class which has the maximum predicted probability and called pseudo label. The pseudo labels are used as if they were true labels. In contrast, \cite{laine2016temporal} introduce the $\Pi$ model exploiting the  stochasticity of the prediction function itself (i.e. the prediction model can produce different outputs for the same input) to apply consistency regularization to standard supervised learning framework. $\Pi$ model achieves this by adding a loss term to encourage the difference between a network's output for different passes of the same image to be small. This is shown to be efficient and effecitve on semi-supervised learning. However, as $\Pi$ model relies on a potentially unstable ``target” prediction, which can rapidly change during the course of training and the ``target" prediction can be very noisy, the training process can be unstable. To tackle the difficulty with $\Pi$ model, \cite{tarvainen2017mean} propose Mean Teacher which exploits an exponential average update strategy to update a teacher network for ``target" prediction. In Mean Teacher, the teacher network made via exponential average over the student network is supposed to include more reliable stochastic information and thus the ``target" prediction is more confident. Similarly, \cite{berthelot2019mixmatch} also consider adding the consistency regularization to the network. The most distinction between the proposed MixMatch method and existing consistency regularization based methods (e.g., $\Pi$ model and mean teacher) is, MixMatch average the predictions of different augmentations and sharpen them to form the pseudo labels for the unlabeled images and exploiting the MixUp \cite{zhang2018mixup} to augment both the labeled and unlabeled images. With the labeled guessing and MixUp techniques introduced in the MixMatch, the semi-supervised learning performance on two popular image classification datasets is significantly boosted. 
Different from $\Pi$ model and mean teacher replying on the stochasticity inside the network itself, \cite{miyato2018virtual} develop the Virtual Adversarial Training (VAT) which directly approximates a tiny perturbation radv added to the input which would most signiﬁcantly affect the output of the prediction model. 

% /***weihong adding reviews of label propagation approaches here***/

\noindent \textbf{Semi-supervised regression.}
Apart from the success of semi-supervised learning on classification problem, some advance on regression are achieved in recent years. \cite{jean2018semi} have adapted existing label propagation, VAT \cite{miyato2018virtual} and Mean Teacher \cite{tarvainen2017mean} to be suitable for regression problem under the semi-supervised setting. Differen from these methods, \cite{jean2018semi} proposed a deep kernel learning based approach for semi-supervised learning by adding a loss term in the posterior regularization framework, which aims at minimizing predictive variance of unlabeled data.

Different from these methods for both classification or regression tasks, our proposed method aims at learning the model to automatically and more correctly label unlabeled images. Instead of directly use the current function/model to predict the ``targets" or pseudo labels for unlabeled data, we consider exploiting the supervision signal from the validation data to correct those wrong/noisy ``targets"/pseudo labels for unlabeled data. This enables our method to train the network with more reliable generated supervision signals of unlabeled data and thus boosts the semi-supervised leanring performance on both the classification and regression tasks.

\noindent \textbf{Meta-learning.}
Meta learning has emerged in recent years and is firstly proposed for few shot learning where meta learning enables the few shot learner to be quickly adapted to new tasks with only few examples. \cite{andrychowicz2016learning,finn2017model} propose methods learning gradient through gradient to train a model which has a strong generalization ability to unseen test data and can be easily adapted to new/unseen tasks. \cite{sung2018learning} introduces the relation network to learn an additional metric such that the learned model's feature representation can be generalized for unseen data and unseen tasks. In addition to few shot learning, it is shown that meta learning has a strong ability on hyper-parameter learning, which is known as automatic learning. \cite{ren2018learning} adopt the meta learning to learn the weight of samples to tackle the sample imbalance problem. \cite{lorraine2018stochastic,mackay2019self} exploit the meta learning for automatically learning the hyper-parameters of the deep neural networks. Despite those advance on aforementioned topics, meta learning has been successfully applied on unsupervised learning \cite{hsu2018unsupervised} and semi-supervised learning for few shot learning \cite{ren2018meta}. \cite{ren2018meta} adapts the prototypical network to use unlabeled examples when producing prototypes, enabling the prototypical network to exploit those unlabeled data to assist few shot classification. Different from these methods, we mainly focus on developing meta learning approach for general classification and regression problem. Our method is learned to more correctly label unlabeled image to assist the training of deep neural network. Also, our method is suitable for both classification and regression tasks.



\begin{figure}[ht]
	\begin{subfigure}{1.0\textwidth}
		\centering
		% include first image
		\includegraphics[width=.95\linewidth]{./figures/ToyMoons.pdf}  
		\caption{Results on Moons test data}
		\label{fig:MoonsTest}
	\end{subfigure}
	\begin{subfigure}{1.0\textwidth}
		\centering
		% include second image
		\includegraphics[width=.95\linewidth]{./figures/ToyMoonsUn.pdf}  
		\caption{Results on Moons unlabeled data}
		\label{fig:MoonsUn}
	\end{subfigure}
	\caption{Results on Moons}
	\label{fig:moons}
\end{figure}



% !TEX root = main.tex

\begin{figure*}[t]
	% \vspace{-0.2cm}
		\centering
		% include first image
		\includegraphics[width=.9\linewidth]{./figures/diagram.pdf}  
		\vspace{-.3cm}
		\caption{Computation graph of (a) consistency based semi-supervised learning and (b) our algorithm on imputing unlabeled samples in a deep neural network. Note that the illustration shows three instances of the same network and our method uses a single neural network. Best seen in color.}
		\label{fig:diagram}
	\end{figure*}
	
	\section{Preliminaries for SSL with consistency regularization}\label{sec:sslreview}
	% \subsection{Semi-supervised learning with consistency regularization}\label{sec:sslreview}
	Consider a dataset $\mathcal{D}$ of $N$ samples $\{(\bx_1,\by_1),(\bx_2,\by_2),\dots,(\bx_{N},\by_{N})\}$ where each sample $\bx$ is labelled with $\by$.
	The dataset is further split into a training $\mT$ and hold-out set $\mH$ with $|\mT|$ and $|\mH|$ samples respectively.
	We also have a set of unlabeled samples $\mU=\{\bx^{u}\}_{i=1,\dots, |\mU|}$.
	Our goal is to learn $\Phi_\theta$, a model (\eg a deep neural network) with parameters $\theta$ to correctly predict label of an unseen sample $\bx$ as $\by = \Phi_\theta(\bx)$.
	In the supervised case, we aim to minimize the expected loss on the training set:
	\begin{equation}\label{eq:costT}
	C^{\mT}=\sum_{\bx,\by\in \mT} \ell(\Phi_\theta(\bx),\by)
	\end{equation} where $\ell$ is a task specific loss, such as a soft-max followed by a cross-entropy loss for classification or squared loss for regression tasks.
	
	We are also interested in exploiting the information in the unlabeled samples.
	As their ground-truth labels are not available, many recent semi-supervised methods~\cite{lee2013pseudo,tarvainen2017mean,berthelot2019mixmatch,sohn2020fixmatch} employ a regularization term on the unlabeled samples that encourages the model to produce consistent predictions when its inputs are perturbed.
	In the context of image classification, commonly applied perturbations include geometric transformations (rotation, cropping, scaling) and color jittering.
	
	Without loss of generality, the regularization term or \emph{consistency loss}~$\ell^u$ can be written as a function that computes the difference (defined by a separate function $d$) between the output of the network $\Phi_\theta$ for a (transformed) unlabeled sample $\bx^u$ and an imputed label $\bz^{(\bx^u)}$
	\[
	\ell^u(\bx^u, \bz^{(\bx^u)}; \Phi_\theta) = d(\Phi_\theta(T_{\eta}(\bx^u)),\bz^{(\bx^u)}),
	\]
	with $T_\eta$ being a random transformation (perturbation) on $\bx$ parameterized by $\eta$; common choices of $d$ include cross-entropy and Euclidean distance, as further discussed below. The empirical loss on the unlabeled set is then
	\begin{equation}\label{eq:costU}
	C^{\mU}(Z)=\sum_{\bx^u\in \mU}
	\ell^u(\bx^u, \bz^{(\bx^u)}; \Phi_\theta).
	%\ell^u(\Phi_\theta(T_{\eta}(\bx^u)),\bz^{(\bx^u)}),
	\end{equation} where $Z$ is the set that contains the imputed labels for  $\bx^u\in\mU$. 
	The imputed labels can further be generally defined as $\bz^{(\bx^u)} = \psi(\bx^u)$ for an imputing function $\psi$.
	As an example, we can let $\psi=\Phi_\theta(T_{\eta'}(\bx^u))$ such that $\bz^{(\bx^u)}$ is obtained by computing the network's output for another random transformation of the sample $\bx^u$.
	In this case, minimizing $C^{\mU}$ encourages the network to produce predictions that are invariant to the transformations used.
	We briefly review commonly used imputing functions $\psi$ and difference functions $d$ in the following:
	%Below we review commonly used $\psi$ and $\ell^u$ in the literature.
	
	% \vspace{0.05cm}
	% \noindent \textbf{Pseudo-label (PL) \cite{lee2013pseudo}} imputes the labels for a given unlabeled sample $\bx^u$ as follows: it first generates a soft-label by computing the network output, picks the class with the maximum predicted probability, and then generates an one-hot ``pseudo-label'' vector where all the entries are zero for all categories but the maximum one, \ie $\bz^{(\bx^u)}=\argmax\left(\Phi_\theta(T_{\eta'}(\bx^u))\right)$ where $\eta'$ is a random transformation.
	% The authors use the cross-entropy loss for $d$ to train their model on the unlabeled samples which encourages the network's output not only to be invariant to jittering but also to be confident (\ie low-entropy).
	
	\vspace{0.05cm}
	\noindent \textbf{Mean-teacher (MT) \cite{tarvainen2017mean}} involves two deep neural networks, denoted as student and teacher, where the weights of the teacher model $\theta'$ are an exponential moving average of the student model's weights $\theta$. 
	Formally, at training iteration $t$, $\theta'_{t}=\alpha \theta'_{t-1}+ (1-\alpha)\theta_{t}$ where $\alpha$ is a smoothing coefficient hyperparameter. The labels for unlabeled samples are imputed with the teacher model: $\psi(\bx^u)=\Phi_{\theta'}(T_{\eta'}(\bx^u))$, and 
	$d$ is the Euclidean distance between predictions of the two models so the consistency loss $\ell^u = \lvert\lvert \Phi_\theta(T_{\eta}(\bx^u))-\bz^{(\bx^u)}\rvert\rvert^2$.
	In this case, the student is trained to not only be robust to various transformations but also to be consistent with the teacher.
	%\[
	%C^{\mU}_{\text{MT}} = \sum_{\bx \in \mU}\lvert\lvert \Phi_\theta(\texttt{augment}(\bx,\eta))-\bz\rvert\rvert^2
	%\] where $\bz=\Phi_\theta(\texttt{augment}(\bx,\eta'))$.
	
	\vspace{0.05cm}
	\noindent \textbf{MixMatch (MM) \cite{berthelot2019mixmatch}} imputes labels by applying a sharpening function $\psi(\bx^u)=\texttt{sharpen}\left(\frac{1}{K}\sum_{i=1}^{K}\Phi_{\theta}(T_{\eta_i}(\bx^u)),\beta\right)$
	% \[
	% \psi(\bx^u)=\texttt{sharpen}\left(\frac{1}{K}\sum_{i=1}^{K}\Phi_{\theta}(T_{\eta_i}(\bx^u)),\beta\right)
	% \] 
	where \texttt{sharpen} is a softmax operator that takes in the averaged prediction over $K$ augmentations of $\bx^u$ and $\beta$ is the temperature hyperparameter.
	% The authors show that such a label generation strategy produces better labels
	Similar to MT, MM also uses an Euclidean distance for $d$.
	%\[
	%C^{\mU}_{\text{MM}} = \sum_{\bx \in \mU} \lvert\lvert\Phi_\theta(\bx,\eta)-\bz\rvert\rvert^2.
	%\]
	Note that MM also uses a recent augmentation strategy, MixUp \cite{zhang2018mixup} that mixes both labeled and unlabeled examples with label guesses as a transformation.
	We refer the interested reader to \cite{berthelot2019mixmatch} for more details.
	
	\vspace{0.05cm}
	\noindent \textbf{FixMatch (FM) \cite{sohn2020fixmatch}} imputes the labels for a given unlabeled sample $\bx^u$ as follows: it first generates a soft-label by computing the network output for an augmentation of the unlabeled sample, picks the class with the maximum predicted probability, and then generates an one-hot ``pseudo-label'' vector where all the entries are zero for all categories but the maximum one, \ie $\bz^{(\bx^u)}=\argmax\left(\Phi_\theta(T_{\eta'}(\bx^u))\right)$ where $\eta'$ is a random transformation. 
	The authors employ the cross-entropy loss function for $d$ on the network output of a ``strong'' augmentation (\eg RandAugment \cite{cubuk2019randaugment}) of the unlabeled sample and its imputed label.
	This strategy encourages the learned model to be invariant to the strong jittering.
	% The authors use the cross-entropy loss for $d$ to train their model on the unlabeled samples which encourages the network's output not only to be invariant to jittering but also to be confident (\ie low-entropy).
	
	
	With the imputed labels, model parameters $\theta$ can then be determined by minimizing a linear combination of the two loss functions weighted by $\lambda$
	\begin{equation}
	%\theta^{\ast}(\bz) =\arg\min_{\theta} \; \sum_{\bx,\by\in \mT} \ell(\Phi_\theta(\bx),\by)+\lambda \sum_{\bx^u\in \mU} \ell^u(\Phi_\theta(T_{\eta}(\bx^u)),\bz)
	\theta^{\ast}(Z) =\arg\min_{\theta} \; C^{\mT}+\lambda C^{\mU}(Z).
	\label{eq:opt1}
	\tag{OPT1}
	\end{equation}
	Next we consider the network parameters as a function of the imputed labels and parameterize $\theta^{\ast}$ by $Z$, as the optimum solutions to \ref{eq:opt1} depend on the set of imputed labels used.
	
	\input{alg}
	
	\section{Method}\label{s:method}
	% \vspace{-0.2cm}
	% \subsection{Learning to impute}
	State-of-the-art methods focus on engineering imputation strategies to obtain better generalization performance when training models with
	\ref{eq:opt1} \cite{laine2016temporal,tarvainen2017mean,berthelot2019mixmatch}.
	%CS: update this citation?
	However, this process is highly manual 
	%and computationally inefficient 
	as it relies on trial and error.
	We instead propose a more direct approach, \emph{to learn $Z$ from data} such that $\theta^{\ast}(Z)$ generalizes well. 
	
	To this end, we treat $Z$ as \emph{learnable} parameters and learn them using the following bi-level optimization framework, where we want to find imputed labels $Z$ that give us the best performance on a hold-out set when parameters are determined by \ref{eq:opt1} with these labels:
	\begin{equation}\label{eq:opt2}
	\min_{Z} \; C^{\mH}(\theta^{\ast}) \;\;  \text{subject to} \;\; \theta^{\ast}(Z)  =\arg\min_{\theta}  \; C^{\mT}+\lambda C^{\mU}(Z).
	\tag{OPT2}
	\end{equation}
	\begin{comment}
	Solving \ref{eq:opt2} requires a nested loop optimization where the inner loop optimizes for $\theta$ over the samples of $\mT$ and $\mU$ by using \ref{eq:opt1}, and outer one optimizes over $\mH$ by using \ref{eq:opt2} given the result of \ref{eq:opt1}.
	As running the inner loop multiple times can be prohibitively expensive in case of large datasets, here we propose an online approximation for the proposed optimization in \ref{eq:opt2}.
	\end{comment}
	\noindent \textbf{Solving \ref{eq:opt2}.}
	Standard approaches to solving \ref{eq:opt2} employ implicit differentiation, which involves solving the inner optimization for $\theta^*$ and an associated linear system to high precision to recover the gradient for $Z$ (see \cite{Do2008,samuel2009learning,domke2012generic} for details). However, this approach is challenging to implement in practice for deep neural networks, due to the high computational cost of training networks to convergence even for a single gradient; in the event that solutions are not obtained with sufficient precision, the resulting gradients become too noisy to be useful \cite{domke2012generic}.
	
	As such, we adopted the back-optimization approach of \cite{domke2012generic} which instead defines $\theta^*$ as the result of an incomplete optimization. Formally, %As such, we consider the case where the minimization of the inner loop is possibly incomplete as in \cite{domke2012generic}:
	\begin{equation}\label{eq:opt1a}
	\theta^{\ast}(Z) =\texttt{opt-alg}_{\theta} \; (C^{\mT}+ \lambda C^{\mU}(Z))
	\end{equation} where \texttt{opt-alg} denotes a specific optimization procedure with a fixed number of steps, which sets a trade-off between accuracy and computational load.
	We wish to solve \ref{eq:opt2}, even in cases where the optimization in \cref{eq:opt1a} has not converged.
	As we experiment with deep neural networks, we use multiple steps of SGD for \texttt{opt-alg} for simplicity; it is also possible to employ other optimizers in this framework (like SGD with momentum). We can then compute the gradient over $Z$ using automatic differentiation by explicitly unrolling the optimization steps over $\theta^*$.
	
	\vspace{0.05cm}
	\noindent \textbf{Algorithm.} 
	\Cref{fig:diagram} depicts an overview of our algorithm.
	Unlike recent SSL work that optimize a consistency loss ($C^{\mU}$) to update its parameters $\theta$ (\ie step 1, 2 in \Cref{fig:diagram}(a)) for each unlabelled image $\bx^u$ and its imputed label $\bz^{(\bx^u)}$, our method utilizes the update to produce an intermediary model $\theta^\ast$ which is evaluated on a hold-out set (\ie step 1, 2, 3 in \Cref{fig:diagram}(b)), then computes an update for $\theta$ by unrolling the gradient graph over $\theta^\ast$ (\ie step 4, 5, 6 in \Cref{fig:diagram}(b)).
	
	
	
	We also give a more detailed description of the optimization procedure in Alg.~\ref{algorithm:option12}.
	Given $\mT$, $\mU$ and $\mH$, we first randomly sample a mini-batch from each set, denote them as $B^{\mT}$, $B^{\mU}$ and $B^{\mH}$ respectively at each iteration $t$.
	We then initialize $\bz$ for the unlabeled batch $B^{\mU}$ by using $\psi(\cdot)$.
	Note that we evaluate our method for various $\psi$ selection in \cref{s:exp}.
	Next we optimize the model parameters for $C^{\mT}+\lambda C^{\mU}$ by using the Adam optimizer~\cite{kingma2014adam} and obtain $\hat{\theta}^t$. We re-impute $\bz$ with $\hat{\theta}^t$ and run the inner-loop by minimizing $C^{\mT} + C^{\mU}$, obtaining $\theta^{\ast}$ for outer-loop optimization.
	
	For the inner-loop, we use a SGD optimizer with fixed number of steps for \texttt{opt-alg} in \cref{eq:opt1a} to obtain $\theta^{\ast}$ by using \cref{eq:opt1a}.
	For one step SGD, \texttt{opt-alg} is simply given by $\theta^{\ast} = \hat{\theta}^t - \eta_{\theta} \nabla_\theta (C^{\mT}+ C^{\mU})$ where $\nabla_\theta$ is the gradient operator and $\eta_{\theta}$ is the learning rate.
	
	For the outer-loop optimization, we wish to find $Z$ that minimizes $C^{\mH}(\theta^{\ast})$ in \ref{eq:opt2}.
	Now we apply the chain rule to the objective function of \ref{eq:opt2} to obtain
	\begin{equation}\label{eq:updopt1}
	%\frac{\partial{C}^H}{\partial \bz} = \sum_{\bx\in B^\mH_t} \frac{\partial \ell(\Phi_{\theta^{\ast}}(\bx), \by)}{\partial \theta^{\ast}}\cdot \left(\frac{\partial \theta^t}{\partial \bz}- \eta \nabla_{\bz}\nabla_\theta C^{\mU} \right)
	\frac{\partial{C}^\mH}{\partial \bz} = 
	\frac{\partial C^{\mH}}{\partial \Phi_{\theta^{\ast}}} \frac{\partial \Phi_{\theta^{\ast}}}{\partial \theta^{\ast}} \frac{\partial \theta^{\ast}}{\partial \bz}
	\tag{V1}
	\end{equation} where ${\partial \theta^{\ast}}/{\partial \bz}={\partial \hat{\theta}^t}/{\partial \bz}- \eta_{\theta} \nabla_{\bz}\nabla_\theta C^{\mU}$ when \texttt{opt-alg} is an one-step SGD optimizer.
	We then use the gradient (${\partial{C}^\mH}/{\partial \bz} $) for \ref{eq:updopt1} to update $\bz$, obtain $\hat{\bz}$ and optimize the model parameters to minimize $C^{\mU}(\{\hat{\bz}\})$. 
	
	Thus far, we have treated $\bz$ as learnable parameters and initialize them with the imputing function $\psi$.
	Alternatively, $\bz$ can be defined as the output of $\psi$ which is typically a function of $\Phi$ (see \cref{sec:sslreview}) and thus also parameterized by $\theta$.
	In other words, the imputing process can also be improved by optimizing $\theta$ as follows:
	\vspace{-.1cm}
	\begin{equation}\label{eq:updopt2}
	\frac{\partial{C}^\mH}{\partial \hat{\theta}^{t}} = 
	\frac{\partial C^{\mH}}{\partial \Phi_{\theta^{\ast}}} \frac{\partial \Phi_{\theta^{\ast}}}{\partial \theta^{\ast}} \frac{\partial \theta^{\ast}}{\partial \psi }
	\frac{\partial \psi}{\partial \hat{\theta}^{t} }
	\tag{V2}
	\end{equation} 
	In this case, the gradient ${\partial{C}^\mH} / {\partial \hat{\theta}^{t}}$ is directly applied to update $\hat{\theta}^{t}$.
	We evaluate both V1 and V2 variants in our experiments.
	% We denote the variations in \cref{eq:updopt1} and \cref{eq:updopt2} as ``V1'' and ``V2'' respectively.
	
	
	\vspace{0.05cm}
	\noindent \textbf{Computational considerations.} Training our method using V1 and V2 involves 2 and 1 extra back-propagation step respectively as well as a second-order derivative computation on unlabeled samples for both, which is the computational bottleneck. We expect that replacing this computation by a more efficient approximation of second-order derivatives (\eg \cite{mehra2019penalty}) will enable our approach to scale to larger datasets such as ImageNet.
	
	
	\vspace{0.05cm}
	\noindent \textbf{Analysis.} We attempt to provide insight into the behavior of our algorithm by analytically computing the update rule \ref{eq:updopt1} for an one-layer network in the semi-supervised binary classification setting. Here, $\Phi_{\theta}(\bx)=\sigma(\theta^\top \bx)$ where $\sigma$ is the sigmoid function.
	In this case, for a given unlabeled sample $\bx^u$, its associated imputed label $z$ and a set of hold-out samples, the update rule \ref{eq:updopt1} for $z$ is: 
	% $\frac{\partial C^{\mH}}{\partial z} =\eta_{\theta}\sum_{\bx,y\in\mH}(\sigma({\theta^*}^\top\bx)-y)\bx^\top\bx^u$
	% \begin{comment}
	\begin{equation}
	\begin{aligned}
	\frac{\partial C^{\mH}}{\partial z} &=\eta_{\theta}\sum_{\bx,y\in\mH}(\sigma({\theta^*}^\top\bx)-y)\bx^\top\bx^u
	\end{aligned}
	\end{equation}\label{eq:sod}
	% \end{comment}
	where $\theta^{\ast}$ is obtained with \ref{eq:opt1}, $y\in\{0,1\}$, $\eta_\theta$ is the learning rate for $\theta$.
	The update rule is proportional to the similarity (dot product) between the unlabeled and hold-out samples, and to the loss between the prediction and the ground-truth labels. Intuitively, the algorithm updates the imputed label towards the majority class of the incorrectly predicted samples on the hold-out set, weighted by the similarity of the unlabeled sample to the respective hold-out sample; correctly predicted hold-out samples do not contribute to the update. 
	We provide the details of the derivation for binary classification and also regression in the supplementary.
	
	
	\vspace{0.05cm}
	\noindent \textbf{Approximation.}
	As discussed above, the computational bottleneck of our method is the computation of an Hessian. The dimension of the Hessian can be millions when we use a deep network. To enable our method to be scalable to large networks and large datasets, we consider to approximate the hessian computation.
	
	
	Normally, a deep network is composed of a large feature extractor and a linear classifier. In \Cref{eq:sod}, we show the update rule of a linear classifier performing classification and regression and the update rule is proportional to the similarity (dot product) between the unlabeled and hold-out samples, and to the loss between the prediction and the ground-truth labels. Thus, when we use a deep network, we can approximate $\frac{\partial C^{\mH}}{\partial z}$ using the similarity between the features of the unlabeled and hold-out samples:
	\begin{equation}
	\begin{aligned}
	\frac{\partial C^{\mathcal{H}}}{\partial z} &\approx \eta_{\theta}\sum_{\bx,y\in\mathcal{H}}(\Phi_{\theta^{\ast}}(\bx)-y)\texttt{vec}(\Phi_{\theta^{\ast}_{f}}(\bx))^\top\texttt{vec}(\Phi_{\theta_{f}}(\bx^u))
	\end{aligned}
	\end{equation}
	where $\theta$ is a deep neural network, which consists of feature encoder $\theta_f$ and the classifier $\theta_c$. 
	$\Phi_{\theta^{\ast}}(\bx)$ is the prediction of an hold-out sample $\bx$ by $\theta^{\ast}$ and $\Phi_{\theta^{\ast}_{f}}(\bx)$ is the feature of $\bx$ by the feature encoder $\theta^{\ast}_f$. $\texttt{vec}(\cdot)$ is the vectorization operator. 
	 
	
	%While our implementation is purposed only for proof-of-concept, we plan to replace the bottleneck with a more efficient 2nd derivatives approximation (\eg \cite{mehra2019penalty}) and apply our method to large-scale datasets (\eg ImageNet) in the future.
	
	% In addition, we also show that our method is related to the well-known label propagation of \citep{xiaojin2002learning} .
	

==> tab_conv_cifar.tex <==
% !TEX root = main.tex
% \begin{table*}[h]
% 	\vspace{-.1cm}
% 	\centering
%   	\resizebox{\textwidth}{!}{  
% 		\begin{tabular}{lccccc|ccccc}
			
% 			 & \multicolumn{5}{c}{CIFAR-10} & \multicolumn{5}{c}{CIFAR-100} \\
% 			\toprule
% 			\#labels       & 250 & 500 & 1000 & 2000 & 4000 & 1000 & 2000 & 3000 & 4000 & 5000 \\
% 			\midrule
% 			SL             & 57.95 & 46.06 & 37.21 & 25.32 & 19.03 & 82.32 & 72.08 & 65.06 & 61.81 & 57.90\\
% 			PL             & 45.19 & 36.58 & 27.19 & 22.12 & 17.5 & 76.30 & 67.32 & 60.76 & 56.53 & 53.82\\
% 			PL+V1 & 43.74 & 35.76 & 26.46 & 21.14 & 16.81 & 75.67 & 66.03 & 60.36 & 56.28 & 53.01\\
% 			PL+V2 & {\bf 42.51} & {\bf 35.43} & {\bf 26.38} & {\bf 20.74} & {\bf 16.65} & {\bf 75.12} & {\bf 64.37} & {\bf 59.03} & {\bf 56.00} & {\bf 52.79}\\
% 			\bottomrule
% 		\end{tabular}%
% 	}
% 		\caption{Error percentage \wh{of testing set} on CIFAR-10 and CIFAR-100.}
% 		\label{tab:cifar}%
% 		\vspace{-.1cm}
% \end{table*}%

\begin{table}[h]
	\vspace{-.1cm}
	\centering
  	\resizebox{1.0\textwidth}{!}
  	{  
		\begin{tabular}{lccccc|ccccc}
			
			 & \multicolumn{5}{c}{CIFAR-10} & \multicolumn{5}{c}{CIFAR-100} \\
			\toprule
			\#labels       & 250 & 500 & 1000 & 2000 & 4000 & 500 & 1000 & 2000 & 3000 & 4000  \\
			\midrule
			SL             & 57.95 & 46.06 & 37.21 & 25.32 & 19.03 & 88.23 & 82.32 & 72.08 & 65.06 & 61.81 \\
			PL             & 45.19 & 36.58 & 27.19 & 22.12 & 17.5 & 85.00 & 76.30 & 67.32 & 60.76 & 56.53 \\
			PL+V1 & 43.74 & 35.76 & 26.46 & 21.14 & 16.81 & 84.41 & 75.67 & 66.03 & 60.36 & 56.28 \\
			PL+V2 & {\bf 42.51} & {\bf 35.43} & {\bf 26.38} & {\bf 20.74} & {\bf 16.65} & {\bf 84.04}& {\bf 75.12} & {\bf 64.37} & {\bf 59.03} & {\bf 56.00} \\
			\bottomrule
		\end{tabular}%
	}
	\vspace{0.1cm}
		\caption{Classification error (\%) \wh{on the test sets} of CIFAR-10 and CIFAR-100.}
		\label{tab:cifar}%
		\vspace{-.5cm}
\end{table}%

